Joint mean and covariance estimation with unreplicated matrix-variate data

It has been proposed that complex populations, such as those that arise in genomics studies, may exhibit dependencies among observations as well as among variables. This gives rise to the challenging problem of analyzing unreplicated high-dimensional data with unknown mean and dependence structures. Matrix-variate approaches that impose various forms of (inverse) covariance sparsity allow flexible dependence structures to be estimated, but cannot directly be applied when the mean and covariance matrices are estimated jointly. We present a practical method utilizing generalized least squares and penalized (inverse) covariance estimation to address this challenge. We establish consistency and obtain rates of convergence for estimating the mean parameters and covariance matrices. The advantages of our approaches are: (i) dependence graphs and covariance structures can be estimated in the presence of unknown mean structure, (ii) the mean structure becomes more efficiently estimated when accounting for the dependence structure among observations; and (iii) inferences about the mean parameters become correctly calibrated. We use simulation studies and analysis of genomic data from a twin study of ulcerative colitis to illustrate the statistical convergence and the performance of our methods in practical settings. Several lines of evidence show that the test statistics for differential gene expression produced by our methods are correctly calibrated and improve power over conventional methods.

==> proofmain.tex <==
\section{Proof sketch of Theorem 1} 
\label{sec::ProofThm1}
\begin{proofof2} 
Let $\BFixed \in \mathbb{R}^{n \times n}$ denote a fixed positive
definite matrix. Let $D$ be as defined as in \eqref{meanMatrixTwoGroups}.  Define $\DeltaFixed = \BFixed^{-1} - B^{-1}$ and
\begin{equation} \label{def:Omega}
\Omega = (D^T B^{-1} D)^{-1} \text{ and } \OmegaFixed = (D^T \BFixed^{-1} D)^{-1}.
\end{equation}
Note that we can decompose the error for all $j$ as
\begin{equation} \label{GLSDecompTriangleIneq}
  \lVert \widehat{\beta}_j(\BFixed^{-1}) - \beta_j^* \rVert_2
    \leq \lVert \widehat{\beta}_j(B^{-1}) - \beta_j^* \rVert_2 + \lVert \widehat{\beta}_j(\BFixed^{-1}) - \widehat{\beta}_j(B^{-1}) \rVert_2 =: \text{I} + \text{II}.
\end{equation}
We will use the following lemmas, which are proved in subsections
\ref{sec::rateBetaHatBHatinvBetaHatBinv} 
and \ref{sec::rateBetaHatBinvBetaStar}, to bound these two terms on the right-hand side, respectively.
\begin{lemma} \label{HansonWrightBetaBinvBetaStar}
Let $\mathcal{E}_2$ denote the event
\begin{equation} \label{eventE2}
  \mathcal{E}_2 = \left\{ \lVert \widehat{\beta}_j(B^{-1}) - \beta_j^* \rVert_2 \leq s_{n, m} \right \},  \quad \text{with} \quad s_{n, m} = C_3 d^{1/2} \sqrt{\frac{\log(m) \lVert B \rVert_2}{n_{\min}}}.
\end{equation}
Then $P(\mathcal{E}_2) \geq 1 - 2 / m^d$.
\end{lemma}
\begin{lemma} \label{BetaBtildeBetaBStarHansonWright}
Let $\BFixed \in \mathbb{R}^{n \times n}$ denote a fixed matrix such that $\BFixed \succ 0$.  Let $X_j \in \mathbb{R}^n$ denote the $j$th column of $X$, where $X$ is a realization of model (\ref{modelMeanCov}).  Let $\mathcal{E}_3$ denote the event
\begin{equation}
\mathcal{E}_3 = \left \{  \lVert \widehat{\beta}_j(\BFixed^{-1}) - \widehat{\beta}_j(B^{-1}) \rVert_2 \leq t_{n, m} \right\}, \quad \text{ with} \quad t_{n, m} = \widetilde{C} n_{\min}^{-1/2} \lVert \DeltaFixed \rVert_2.
\end{equation}
for some absolute constant $\widetilde{C}$.  Then $P(\mathcal{E}_3) \geq 1 - 2 / m^d$.
\end{lemma}
The proof of \eqref{rateBetaHatFixedB1} follows from the union bound $P(\mathcal{E}_2 \cap \mathcal{E}_3) \geq 1 - P(\mathcal{E}_2) - P(\mathcal{E}_3) \geq 1 - 4 / m^d$. Next we prove \eqref{rateGammaHatFixedDelta}. Let $r_{n, m} = s_{n, m} + t_{n, m}$, as defined in \eqref{rateBetaHatFixedB1}, and let $\delta = (1, -1) \in \mathbb{R}^2$. 
Then 
\[ 
	| \widehat{\gamma}_j(\BinvFixed) - \gamma_j | = \left | \delta^T \left( \widehat{\beta}_j(\BinvFixed) - \beta_j^* \right) \right | \leq \lVert \delta \rVert_2 \lVert \widehat{\beta}_j(\BinvFixed) - \beta_j^* \rVert_2 = \sqrt{2} \lVert \widehat{\beta}_j(\BinvFixed) - \beta_j^* \rVert_2, 
\] 
where we used the Cauchy-Schwarz inequality.  Hence if $\lVert \widehat{\beta}_j(\BinvFixed) - \beta_j \rVert_2 \leq r_{n, m}$, it follows that $| \widehat{\gamma}_j(\BinvFixed) - \gamma_j | \leq \sqrt{2} r_{n, m}$.  The result holds by applying a union bound over the variables $j = 1, \ldots, m$.
\end{proofof2}
